Policy Search for Model Predictive Control with Application to Agile Drone Flight

Policy Search and Model Predictive Control~(MPC) are two different paradigms for robot control: policy search has the strength of automatically learning complex policies using experienced data, while MPC can offer optimal control performance using models and trajectory optimization. An open research question is how to leverage and combine the advantages of both approaches. In this work, we provide an answer by using policy search for automatically choosing high-level decision variables for MPC, which leads to a novel policy-search-for-model-predictive-control framework. Specifically, we formulate the MPC as a parameterized controller, where the hard-to-optimize decision variables are represented as high-level policies. Such a formulation allows optimizing policies in a self-supervised fashion. We validate this framework by focusing on a challenging problem in agile drone flight: flying a quadrotor through fast-moving gates. Experiments show that our controller achieves robust and real-time control performance in both simulation and the real world. The proposed framework offers a new perspective for merging learning and control.

==> figures/fig.tex <==
% An example of a floating figure using the graphicx package.
% Note that \label must occur AFTER (or within) \caption.
% For figures, \caption should occur after the \includegraphics.
% Note that IEEEtran v1.7 and later has special internal code that
% is designed to preserve the operation of \label within \caption
% even when the captionsoff option is in effect. However, because
% of issues like this, it may be the safest practice to put all your
% \label just after \caption rather than within \caption{}.
%
% Reminder: the "draftcls" or "draftclsnofoot", not "draft", class
% option should be used if it is desired that the figures are to be
% displayed while in draft mode.
%
%\begin{figure}[!t]
%\centering
%\includegraphics[width=2.5in]{myfigure}
% where an .eps filename suffix will be assumed under latex, 
% and a .pdf suffix will be assumed for pdflatex; or what has been declared
% via \DeclareGraphicsExtensions.
%\caption{Simulation results for the network.}
%\label{fig_sim}
%\end{figure}

%
% Note that often IEEE papers with subfigures do not employ subfigure
% captions (using the optional argument to \subfloat[]), but instead will
% reference/describe all of them (a), (b), etc., within the main caption.
% Be aware that for subfig.sty to generate the (a), (b), etc., subfigure
% labels, the optional argument to \subfloat must be present. If a
% subcaption is not desired, just leave its contents blank,
% e.g., \subfloat[].


==> sections/acknowledgment.tex <==
% use section* for acknowledgment
% \section*{Acknowledgment}
% The authors would like to thank...


==> sections/biography.tex <==
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

% \begin{IEEEbiography}{Michael Shell}
% Biography text here.
% \end{IEEEbiography}

% if you will not have a photo at all:
% \begin{IEEEbiographynophoto}{John Doe}
% Biography text here.
% \end{IEEEbiographynophoto}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

% \begin{IEEEbiographynophoto}{Jane Doe}
% Biography text here.
% \end{IEEEbiographynophoto}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}


==> tables/lineargaussian4mpc.tex <==
% An example of a floating table. Note that, for IEEE style tables, the
% \caption command should come BEFORE the table and, given that table
% captions serve much like titles, are usually capitalized except for words
% such as a, an, and, as, at, but, by, for, in, nor, of, on, or, the, to
% and up, which are usually not capitalized unless they are the first or
% last word of the caption. Table text will default to \footnotesize as
% the IEEE normally uses this smaller font for tables.
% The \label must come after \caption as always.
%
%\begin{table}[!t]
%% increase table row spacing, adjust to taste
%\renewcommand{\arraystretch}{1.3}
% if using array.sty, it might be a good idea to tweak the value of
% \extrarowheight as needed to properly center the text within the cells
%\caption{An Example of a Table}
%\label{table_example}
%\centering
%% Some packages, such as MDW tools, offer better commands for making tables
%% than the plain LaTeX2e tabular which is used here.
%\begin{tabular}{|c||c|}
%\hline
%One & Two\\
%\hline
%Three & Four\\
%\hline
%\end{tabular}
%\end{table}


% Note that the IEEE does not put floats in the very first column
% - or typically anywhere on the first page for that matter. Also,
% in-text middle ("here") positioning is typically not used, but it
% is allowed and encouraged for Computer Society conferences (but
% not Computer Society journals). Most IEEE journals/conferences use
% top floats exclusively. 
% Note that, LaTeX2e, unlike IEEE journals/conferences, places
% footnotes above bottom floats. This can be corrected via the
% \fnbelowfloat command of the stfloats package.

% \begin{table}[tp]
% 	\caption{Success Rate}
% 	\centering
% 	\resizebox{0.5\textwidth}{!}{%
%         % \begin{tabular}{p{2.5cm}||p{2.1cm}|p{1.7cm}|p{4cm}|p{1.7cm}|p{1.7cm}|p{1.5cm}|p{1.7cm} }
%         \begin{tabular}{@{}l|c|c|c|c@{}}
%         	\toprule
%         	\\[-0.4em]
%         	No. Gates & Success Rate & Mean & Std. \\ \\[-0.4em]
%         	\hline
%         	\hline
%         	\\[-0.4em]
%         	0 & 100 & 0.0 & 0.1 &  
%         	\bottomrule
%         \end{tabular}
%     }
% \label{tab:success_rate}
% \end{table}

% \begin{itemize}
%     \item 1 Gates, plan T = 1.0, plan dt = 0.05
%     \item 2 Gates, plan T = 2.0, plan dt = 0.05
%     \item 3 Gates, plan T = 3.0, plan dt = 0.05
% \end{itemize}

\begin{table}[!htp]
    \caption{Linear Gaussian Policy for MPC.}
    \label{tab:lineargaussian4mpc}
    \centering
    \begin{tabular}{c|c|ccc|ccc|ccc}
        \toprule
        \multirow{2}{4em}{Approach} 
            & Number   & \multicolumn{3}{c|}{Success Rates} & \multicolumn{3}{c|}{Mean} & \multicolumn{3}{c}{Std.} \\
            & of Gates &   &(\SI{}{\percent})&  &  &(\SI{}{\meter})&  &  &(\SI{}{\meter})& \\
        \midrule
        \multirow{1}{4em}{Random} 
            % & 1 & 0 & - & - & 2.70 &  -   &  -   & 0.47 &  -   & -    \\ %\cline{3-5}
            % & 2 & 0 & 0 & - & 1.41 & 4.48 &  -   & 0.20 & 0.32 & -    \\ 
            & 3 & 0 & 0 & 0 & 2.75 & 3.46 & 3.45 & 0.45 & 0.25 & 0.99 \\
        \midrule
        \multirow{1}{4em}{Heuristic} 
            % & 1 & 100 &  -  & - & 0.15 &  -   &   -  & 0.01 &   -  &  -    \\ 
            % & 2 & 100 & 100 & - & 0.14 & 0.19 &   -  & 0.03 & 0.05 &  -    \\ 
            & 3 & 100 & 0   & 0 & 0.14 & 1.98 & 1.14 & 0.02 & 0.50 & 0.29  \\
        \midrule
        \multirow{1}{4em}{ \textbf{Ours} }
        % & 1 & 100 &  -  &  - & 0.15 &   -  &   -  & 0.01 &  -   & -    \\
        % & 2 & 100 & 100 &  - & 0.08 & 0.19 &   -  & 0.02 & 0.01 & -    \\
        & 3 & 100 & 100 & 94 & 0.17 & 0.21 & 0.30 & 0.04 & 0.06 & 0.15 \\
        % & 4 & 99  & 96  & 61 & 41 & 0.18 & 0.22 & 0.51 & 0.67 & 0.05 & 0.15 & 0.44 & 0.43 \\
        \bottomrule
    \end{tabular}
\end{table}

